GNN-encoder: Learning a Dual-encoder Architecture via Graph Neural Networks for Dense Passage Retrieval

Recently, retrieval models based on dense representations are dominant in passage retrieval tasks, due to their outstanding ability in terms of capturing semantics of input text compared to the traditional sparse vector space models. A common practice of dense retrieval models is to exploit a dual-encoder architecture to represent a query and a passage independently. Though efficient, such a structure loses interaction between the query-passage pair, resulting in inferior accuracy. To enhance the performance of dense retrieval models without loss of efficiency, we propose a GNN-encoder model in which query (passage) information is fused into passage (query) representations via graph neural networks that are constructed by queries and their top retrieved passages. By this means, we maintain a dual-encoder structure, and retain some interaction information between query-passage pairs in their representations, which enables us to achieve both efficiency and efficacy in passage retrieval. Evaluation results indicate that our method significantly outperforms the existing models on MSMARCO, Natural Questions and TriviaQA datasets, and achieves the new state-of-the-art on these datasets.

==> EMNLP 2022/section/conclusion.tex <==
\pdfoutput=1
\section{CONCLUSION}
In this paper, we introduced \gmodel for passage retrieval tasks and demonstrated its effectiveness on MSMARCO, Natural Questions and TriviaQA datasets. 
The existing dual-encoder architecture, although very efficient, ignores interaction during passage (query) encoding due to its independent architecture. 
Therefore we attempted to fuse query (passage) information into passage (query) representations via graph neural networks and maintain online efficiency of the dual-encoder. However, we may retrieve irrelevant passages for queries by dual-encoder when constructing the query-passage graph, which introduces noise in information propagating. Hence we utilize GAT layers and filter gate to reduce the noise, which are proved necessary by our various experiments. In the future, we will explore how to fuse more interaction information into GNN structure.

==> EMNLP 2022/section/exp.tex <==
\pdfoutput=1
\section{Experiments}
\input{table/main_result}

\subsection{Dataset}
\datatitle{MSMARCO}~\cite{nguyen2016ms} is the dataset introduced by Microsoft. 
%It contains 0.5 million queries and 8.8 million passages.
It contains 0.5 million queries that were sampled from Bing search logs, while containing 8.8 million passages that were gathered from Bing's results to real-world queries.
% Based on this dataset, the passage ranking task is aimed to recalling passages that can answer the question from a collection of 8.8 million passages.
% The training data is labeled by human, while one (or very few) passages are marked as relevant to one query and no passage is labeled as irrelevat.
%\{ each query is associated with sparse relevance judgments of one (or very few) passages marked as relevant and no passages explicitly indicated as irrelevant. \}

\datatitle{Natural Questions} (NQ)~\cite{kwiatkowski2019natural} is a large dataset from open-domain QA, which consists of queries that were issued to the Google search engine by real anonymized, and the collection of passages is processed from Wikipedia.

\datatitle{TriviaQA} (TQA)~\cite{joshi2017triviaqa} contains a set of trivia questions with answers which were originally scraped from the Web.

For both Natural Questions and TriviaQA, we reuse the version released by DPR~\cite{karpukhin2020dense} in our experiments. 
Following previous work, we use mean reciprocal rank (MRR) and recall at top $k$ ranks (R@k) to evaluate the performance of passage retrieval. 

% \subsubsection{Evaluation Metrics}
% Following previous work, we use mean reciprocal rank (MRR) and recall at top $k$ ranks (R@k) to evaluate the performance of passage retrieval. 
% \textbf{MRR} is an internationally common criterion for evaluating search algorithms,
% % where the first result matching, the score is 1, while the second matching score is 0.5, and the n-th matching score is 1/n, if there is no matching sentence score is 0, and the final score is the sum of all scores. 
% and it averages the score that is the reciprocal of the rank at which the first relevant passage is retrieved.
% And the \textbf{Recall} metric is defined as the proportion of questions to which the top $k$ retrieved passages contain answers.

\subsection{Comparison Methods}
To demonstrate the effectiveness of our model, we adopt several state-of-the-art document retrieval models for comparison as follows.

\paratitle{Sparse Retrieval Models}
We first compare our model with sparse passage retrieval models, including traditional retriever BM25~\cite{yang2017anserini}, and three retrievers enhanced by neural networks, DeepCT~\cite{dai2019deepct},  GAR~\cite{mao2020generation} and COIL~\cite{gao2021coil}. 
% DeepCT and COIL employ BERT to learn the term weight. Both doc2query and docTTTTTquery utilize query generation to expand documents.
% while GAR employs generation models to expand queries. UHD-BERT is enhanced by extremely high dimensionality and controllable sparsity.

\paratitle{Dense Retrieval Models}
We compare with several dense passage retrieval models, including DPR~\cite{karpukhin2020dense}, ANCE~\cite{xiong2020approximate}, ColBERT~\cite{khattab2020colbert}, NPRINC~\cite{lu2020nprinc}, RocketQA~\cite{qu2021rocketqa}, PAIR~\cite{ren2021pair} and RocketQAv2~\cite{renrocketqav2}. For PAIR and RocketQAv2, we initialize them with BERT$_{\rm base}$ and reproduce their results on TQA. And we also compare with some pre-training methods, including Condenser~\cite{gao2021condenser} and coCondenser~\cite{gao2021unsupervised}.

\subsection{Implementation Details}\label{sec:id}
For fair comparison with baseline models, the dual-encoder is initialized with ERNIE-2.0 base \cite{zhang2019ernie} 
which is a BERT-like model with 12-layer transformers 
on MSMARCO and NQ, and is initialized with BERT$_{\rm base}$ on TQA. Our initial dual-encoder $M_{de}$ is trained with the batch sizes of $2048 \times 2$ on MSMARCO, and $256 \times 4$ on NQ and TQA. The number of epoch, the rate of linear scheduling warm-up and the learning rate are set to 10, 0.1 and 2e-5, respectively on all datasets.

While jointly training dual-encoder and GNN, we set the learning rate to 2e-6 and 5e-5 for dual-encoder and GNN, respectively, the batch size to $1024 \times 4$ and the number of epoch to 5. Since different network structures are suitable for different learning rate, it is necessary to set them different. We retrieve the top-25 candidate passages for each query by $M_{de}$ to create edge set $\mathcal{E}_{pq}$. For each epoch, we randomly select 5\% of the queries for training while others and their relevant edges for constructing graph. \input{table/trivia_result}
During the inference, we use the query encoder to predict query embeddings, and use FAISS~\cite{johnson2019billion} to index the dense representations of all passages via GNN-encoder.
We implement all experiments with the deep learning framework PyTorch on up to four NVIDIA Tesla A100 GPU (80GB memory).
%The implementation code of \gmodel is based on Huggingface Transformers \cite{wolf2020transformers} and DGL \cite{wang2019deep} with utilizing gradient checkpointing \cite{chen2016training} and Apex to reduce GPU memory consumption if needed.

\subsection{Experimental Results}
The detailed experimental results of passage retrieval tasks on MSMARCO and NQ are shown in Table~\ref{tab:mainR}, while the results of TQA are shown in Table~\ref{tab:triviaR}. We can observe that our model outperforms other fine-tuning methods by a large margin, especially on MRR@10 (+0.5\%), R@50 (+0.5\%) of MSMARCO, R@5 (+1.7\%), R@20 (+1.2\%) of NQ and R@5 (+1.3\%), R@20 (+0.7\%) of TQA. This phenomenon reflects that our model can build better query and passage representations to improve the ability of passage ranking at top ranks, which is due to our interaction between query embeddings and passage embeddings. When compared to pre-training methods like coCondenser, our model still performs better in general on all datasets. Note that pre-training methods are not comparable to our method in practice, but complementary work.



\subsection{Ablation Study}
\input{table/ablation}


We perform an ablation study to investigate where the improvement mainly comes from. We only report the results on NQ which are shown in Table~\ref{tab:ablation}, while the results on MSMARCO and TQA are similar and omitted here due to limited space.

First, we use Eq.(\ref{eq:sim}$\sim$\ref{loss}) to train a dual-encoder without GNN on query-passage graph and compare it with our model to explore how much performance improvement is introduced by GNN.
The performance of our model notably drops in terms of R@5 and R@20 without GNN. 
%, which is comparable to PAIR and RocketQAv2. 
It indicates that our model builds better query and passage embeddings by GNN interaction, which improves the performance at top ranks.

%Dropping positive labeled edges is a widely used method to avoid information leakage in GNN libraries like DGL~\cite{wang2019deep}. 
We use the whole training queries to both construct the graph and train \gmodel at the same epoch and drop edges between training queries and their positive passages to avoid information leakage like DGL~\cite{wang2019deep} instead of MGT Algorithm. 
However, it leads to a considerable drop in performance as shown in Table~\ref{tab:ablation}. We conclude the reason as in-batch negatives information leakage. 
As illustrated in Figure~\ref{fig:attention}, w/o MGT can lead to information leakage, because the passage embeddings will be more inclined to integrate the queries labeled positive in training dataset but ignore potentially relative queries \footnote{If query $q$ is supposed to have positive passage $p$, but for some reason it is not labeled, we consider $q$ to be a potentially relative query of $p$.} (as left attention scores show scores of labeled positive queries are much bigger than the others). 
However, our algorithm can solve this problem, due to queries for training are not used to construct graph in the same training epoch (as right attention scores show scores of potentially relative queries become larger). 
% Second, there is discrepancy between the training and inference process, and inference queries are not contained by graph query node set, while training queries are contained. Therefore, in every epoch, we split the training queries into two parts $Q_g$ and $Q_t$ for constructing the graph and training GNN respectively, which make training queries not in graph node set and make the training and prediction process consistent.

\begin{figure}
     \centering
     \includegraphics[width=1.0\columnwidth]{figs/attention.pdf}
     \caption{
         Attention scores in Eq.(\ref{eq:atention}) for w/o MGT (left) and w/ MGT (right). We illustrate a passage and queries connecting to it in $\mathcal{G}$, and mark labeled positive queries in training dataset and potentially relative queries in {\color{red}red} and {\color{blue}blue}, respectively.
     }
     \label{fig:attention}
\end{figure}

And then, we remove the filter gate in Eq.(\ref{eq:ipe}) and calculate query-interactive passage embeddings directly with a constant $\alpha$, \ie~$h_{p_i}' = \alpha \cdot \widetilde{h_{p_i}} + h_{p_i}$. For a more fair comparison, we searched for $\alpha$ from $0$ to $1$ by setting an equal interval to $0.1$, and release the best result in Table~\ref{tab:ablation} where $\alpha$ is set to $0.2$. However, the best result of replacing filter gate with constant $\alpha$ is still lower than that of filter gate. A potential reason is that the value of $\alpha$ should not be the same for different passages.
%, because some passages may only need to incorporate a small amount of query information, while others need to incorporate more.

We also investigate whether the embeddings of cross encoder as edge features can effectively guide model to learn attention mechanism. As shown from results, the performance slightly drops when we remove the edge features. It indicates that GAT layer can learn how to select information from neighbors by only relying on passage embeddings and query embeddings, but the embeddings of cross encoder help it learn better.

We utilize one GAT layer instead of two layers to examine the effect of two-hop neighbors. As shown in Table \ref{tab:ablation} (w/ one layer), the performance of one layer drops compared to that of two layers. We think that the passages retrieved by a query which are also part of the query information, will complement the query embeddings. That is also the reason why two layers have better performance.

\subsection{Detailed Analysis}\label{DA}
Apart from the above illustration, we also implement detailed analysis on different settings of \modelnospace's training and efficiency.

\paratitle{The number of edges in Graph}
\begin{figure}
    \centering
    \includegraphics[width=1.0\columnwidth]{figs/edges.pdf}
    \caption{
        R@5 (left) and R@20 (right) results of passage retrieval on NQ with different numbers of edges per query node.
    }
    \label{fig:egde}
\end{figure}
% As Figure~\ref{fig:egde} illustrated, we analyze the influence of the number of edges connected to a query node on the experimental results. 
For graph construction in section~\ref{3.2}, the more candidate passages are retrieved, the more edges there will be, which means that more queries connect to a passage and more query information could be incorporated into passage embeddings. 
However, Figure~\ref{fig:egde} indicates that more edges do not bring further performance improvements, because excessive edges might introduce noise that increases the difficulty of model learning and leads to performance drop.

\paratitle{Masked Ratio}
\begin{figure}
    \centering
    \includegraphics[width=1.0\columnwidth]{EMNLP 2022/figs/Beta.pdf}
    \caption{
        R@5 (left) and R@20 (right) results of passage retrieval on NQ with different masked ratios.
    }
    \label{fig:beta}
\end{figure}
In this part, we conduct an experiment to analyze the impact of the masked ratio on retrieval performance. 
As shown in Figure~\ref{fig:beta}, high masked ratio $\beta$ has poor performance, because it causes the discrepancy between the training graph and the inference graph~(the large $\beta$ means a few training queries used to construct graph in a training epoch). 
But it is also not necessary to set $\beta$ too small, since it will bring overhead for frequent constructing graph without any performance improvement~(the small $\beta$ means a few queries used to train which leads to more training epochs).

\input{table/efficiency}
\paratitle{Efficiency} We test the efficiency of our model on a single NVIDIA Tesla A100 80GB GPU for the NQ test set, and record the encoding time per document and retrieval time per query (including query encoding time), as shown in Table \ref{tab:effic}. Since we need to additionally compute query-interactive passage embeddings via GNN, the document encoding time is slightly longer than dual-encoder models. 
% However, the increase is very little compared to the computation time of passage encoder. 
Since query-interactive passage embeddings can be pre-computed offline once obtained from \gmodel, we only need to encode query. Therefore we do not bring additional computation overhead to online retrieval (same as dual-encoder models).

==> EMNLP 2022/section/intro.tex <==
\pdfoutput=1
\section{Introduction}
Large-scale query-passage retrieval is a core task in search systems, which aims to rank a collection of passages based on their relevance with regard to a query. To balance efficiency and effectiveness, existing work typically adopts a two-stage retrieval pipeline~\cite{renrocketqav2,twostageQA}. The first-stage aims to retrieve a subset of candidate passages by a recall model from the entire corpus and the second stage aims to re-rank the retrieved passages. %Since the recall model in the first-stage determines the upper bound of the ranking model performance in the second-stage, a lot of work focuses on improving the recall performance of the first-stage retrieval~\cite{DocumentRankingSeq2Seq,Context-AwareTermImportance}.
In the first-stage retrieval, traditional approaches~\cite{traditionalqa} implemented term-based retriever (e.g. TF-IDF and BM25) by weighting terms based on their frequency, which have limitations on representing semantics of text. Recently, dense passage retrieval is drawing more and more attention in the task of passage retrieval~\cite{karpukhin2020dense}. The underlying idea is to represent both queries and passages as embeddings, so that the semantic relevance can be measured via embeddings similarity. 
With the great success of pre-trained language models (PLMs) such as BERT/RoBERTa~\cite{BERT,RoBERTa} in natural language processing tasks, dense retrieval models parameterized by PLMs is emerging as the new state-of-the-art in a variety of passage retrieval tasks \cite{karpukhin2020dense,xiong2020approximate}. 

Two paradigms based on fine-tuned language models are typically built for retrieval: cross-encoders and dual-encoders. 
%As a typical cross-encoder model, BERT takes the concatenation of the query-passage pair as input and performs a full self-attention calculation across the input tokens. 
Typical cross-encoders need to recompute the representation of each passage in the corpus once a new query comes, which is difficult to deploy in real-world search systems. 
%Though the full self-attention provides rich interaction signals, it brings high computational cost and inference latency since it needs to recompute the representation of each passage in the corpus once a new query comes. As a result, it is usually difficult to deploy a cross-encoder model in real-world search systems. 
In contrast, dual-encoders remove query-passage interaction by representing a query and a passage independently through two separate encoders (Siamese encoders). Hence, passage embeddings can be pre-computed offline, and online latency can be greatly reduced.
Thanks to this advantage, dual-encoders are more widely adopted in real-world applications. 
On the other hand, independent encoding without any interaction causes severe retrieval performance drop due to information loss. To improve the performance of dual-encoders, some efforts have been made to incorporate more complicated structures (i.e., late interaction) such as attention layers~\cite{Humeau2019polyencoder, tang2021Pseudo}, the sum of maximum similarity computations ~\cite{khattab2020colbert}, and the transformer layers~\cite{deformer, dipair} into encoding. 
%Late interaction introduces simple interaction layers before the final prediction layer in order to mitigate information loss in retrieval. Along this line, various strategies have been proposed, such as attention layers~\cite{Humeau2019polyencoder, tang2021Pseudo}, the sum of maximum similarity computations ~\cite{khattab2020colbert}, and the transformer layers~\cite{deformer, dipair}. 
These late interaction strategies bring considerable improvements on retrieval performance but also increase computational overhead. Moreover, interaction information is still neglected in earlier encoding of query and passage.
%though queries and passages finally meet each other in these models, interaction information is still neglected in query and passage encoding.

In this work, we aim to achieve both efficiency and effectiveness in passage retrieval. The key idea is to maintain two independent encoders, and keep as much interaction information as possible in the meanwhile. To this end, we propose a novel approach that explicitly fuses query (passage) information into passage (query) embeddings through a graph neural network (GNN), and name the model \modelnospace. Our model is built upon the dual-encoder, and learns query-interactive passage representations and passage-interactive query representations through a graph neural network. Specifically, given a query set, we retrieve top passages for each query, and form a graph whose nodes are the queries and the passages, and edges reflect correspondence between query-passage pairs (i.e., if a passage is retrieved by the query). 
Then, we initialize the GNN model with the representations of the pre-trained dual-encoder and cross-encoder, and then perform information propagation on the graph.
%by which passage-query (query-passage) interaction and passage-query-passage (query-passage-query) relationship are encoded into the node representations via one-hop neighbors and two-hop neighbors respectively. After that, passage (query) embeddings is defined as the representations of the passage (query) nodes. 
To avoid information leakage, we further design a new training algorithm and name it Masked Graph Training (MGT), in which the query set used for training GNN is no longer used to construct the query-passage graph in each training epoch. 
%Finally, query embeddings are obtained by re-training the dual-encoder with the query-interactive passage representations rather than using the graph representations. This is motivated by efficiency considerations, since running a GNN algorithm online for new queries is costly. Therefore, our method is the same online latency as dual-encoder, due to the passage embeddings could be pre-computed offline. 
Finally, the passage embeddings could be pre-computed offline corresponding to the GNN. 
Thus our model holds the efficiency advantage inherited from the dual structure, and at the same time takes query-passage interaction into account.  


%Propagating information within the graph helps to understand both passage-query (query-passage) interaction through one-hop neighbors and passage-query-passage (query-passage-query) relationship through two-hop neighbors, where the query (passage) can serve as the bridge connecting semantically related passages (queries). Therefore, deep query-passage/passage-passage/query-query interaction signals are captured during query and passage encoding via GNN. 
%Unfortunately, directly applying the whole training query set when constructing query-passage graph and training \gmodel can lead to the problem of over-fitting, because the passage (query) embedding will increasingly tend to fuse the queries (passages) related to it in the training set while ignoring other potentially related queries (passages).
%Thus, we design a graph learning algorithm for passage retrieval and we call it 
%Finally, the ``query-interactive passage embeddings'' and ``passage-interactive query embeddings'' are obtained simultaneously through \gmodel. 
%It's noteworthy to mention that the ``query-interactive passage embeddings'' can be pre-computed offline once obtained from \gmodel . However, the ``passage-interactive query embeddings'' should inference via \gmodel online once a new query comes, which brings high computational cost and inference latency. We further re-train the query encoder according to the passage embeddings without GNN, thereby not only improving the query embeddings' quality but also maintaining the online computation unchanged (same as dual-encoder).

Our contributions can be summarized as follows:
\begin{itemize}
    \item We propose a novel dense retrieval model based on graph neural network techniques that encodes query-passage interaction into query and passage representations without sacrifice on retrieval efficiency.  
    %To the best of our knowledge, it is the first time that interaction has been considered during query and passage encoding for passage retrieval tasks. 
    \item We propose an adaptive Masked Graph Training (MGT) Algorithm for our task to avoid information leakage during GNN training.
    \item Experiments show that our model achieves state-of-the-art performance on MSMARCO, Natural Questions and TriviaQA datasets.
\end{itemize}

==> EMNLP 2022/section/limit.tex <==
\pdfoutput=1
\section*{Limitations}
In this section, we will discuss the limitations of our work, which we consider as two major points: the requirement of more physical memory and utilizing cache passage embeddings as passage node features.

In both training and document encoding process of \gmodel, we need cache passage embeddings of $M_{de}$ ($m$ passage nodes) and embeddings of cross-encoder (($n\times k + m +n$)  edges), which should be calculated and stored in advance. It means that we need to store at least ($(n\times k + 2m + n) \times d$) floating-point numbers, where d is the dimension of BERT base. In practice, the number of passages $m$ is often very large, for example, the NQ dataset has about 20 million passages. Feature compression may be a good solution, but it may lead to performance drop.

As mentioned in Section \ref{3.4}, we utilize cache passage embeddings of $M_{de}$ as passage node features to compute $\widetilde{h_{q_i}}$ in Eq.(\ref{eq:gat1}) instead of recomputing them by passage encoder. It may be not the best approach for joint training dual-encoder and GNN, but it is a more practical way considering efficiency and hardware resources. We have tried to update cache passage embeddings, but it brings very little improvement and increases convergence difficulty.

==> EMNLP 2022/section/method.tex <==
\pdfoutput=1
\section{Methodology}
\subsection{Preliminary}
Given a query $q$, dense retriever is required to retrieve k most relevant passages $\{p_i\}_{i=1}^k$ from a large corpus consisting of hundreds of thousands of passages. For the sake of retrieval efficiency, the dual-encoder architecture is widely adopted, where query encoder $E_Q(\cdot)$ and passage encoder $E_P(\cdot)$ are used to embed query $q$ and passage $p$ into $d$-dimensional vectors, respectively. The similarity between query $q$ and passage $p$ can be computed as the dot product of their vectors:
\begin{equation}\label{eq:sim}
    s(q,p) = E_Q(q)^\mathrm{T}\cdot E_P(p).
\end{equation}

The training objective of the dual-encoder is to learn embeddings of queries and passages to make positive query-passage pairs have higher similarity than the negative query-passage pairs in training data. Hence, the contrastive-learning loss function is adopted for the dual-encoder:
\begin{equation}\label{loss}
     \begin{aligned}
    &L(q,p^+,\{p^-\},s) = \\
    &- \log \frac{e^{s(q,p^+)}}{e^{s(q,p^+)}+\sum_{\{p^-\}}e^{s(q,p^-)}},
    \end{aligned}
\end{equation}
where $q$ and $p^+$ represent query and positive passage, respectively, and $\{p^-\}$ represents the set of negative passages.

In practical retrieval systems, passage embeddings are usually pre-computed offline, while query embeddings are computed by the query encoder in an ad hoc manner. Therefore we can obtain better passage embeddings through a complicated encoder as long as it does not increase the online inference latency.

\subsection{Graph Construction} \label{3.2} We use all the passages $P = \{p_i\}_{i=1}^m$ and training queries 
$Q = \{q_i\}_{i=1}^n$ as nodes to construct our \textbf{query-passage graph}, where $n$ and $m$ denote the number of training queries and passages, respectively. Let $\mathcal{G} = (\mathcal{V},\mathcal{E})$ denote our graph, where $\mathcal{V} = \mathcal{V}_q \cup \mathcal{V}_p$ is a node set and $\mathcal{E} = \mathcal{E}_{pp} \cup \mathcal{E}_{pq} \cup \mathcal{E}_{qq}$ is an edge set. 
$\mathcal{V}_p$ and $\mathcal{V}_q$ denote the passage node set and the query node set, respectively. $\mathcal{E}_{pp}$, $\mathcal{E}_{pq}$, and $\mathcal{E}_{qq}$ denote the edges between passage nodes, between passage nodes and query nodes, and between query nodes, respectively. 
The edge between node $x$ and node $y$ is denoted as $e(x,y)$.

We retrieve the top-k candidate passages $P_i = \{p_{ij}\}_{j=1}^k$ for each query $q_i$ from the corpus by the dual-encoder. We add edges between $q_i$ and each passage $p_{ij}$ in the top-k retrieved passages $P_i$ which may be relevant to $q_i$. These edges compose $\mathcal{E}_{pq}$ (i.e., $\mathcal{E}_{pq} = \{e(q_i,p_{ij})\}_{i=1,j=1}^{n,k}$). Since we can not directly distinguish whether there is relation between the queries and between the passages, we only add self-loops to each passage and query (i.e., $\mathcal{E}_{pp}=\{e(p_i,p_i)\}_{i=1}^m$ and $\mathcal{E}_{qq}=\{e(q_i,q_i)\}_{i=1}^n$). To summarize, our graph $\mathcal{G}$ has a total of $(n+m)$ nodes and $(n\times k + m +n)$ edges.

\paratitle{Node Features} 
We use the dual-encoder to get query embeddings $h_{q_i} = E_Q(q_i)$ and passage embeddings $h_{p_i} = E_P(p_i)$ as our graph node features. 

\paratitle{Edge Features} 
Since the cross-encoder can better capture the interactive information between text pairs, we utilize the embeddings of text pairs $(x,y)$ by the cross-encoder as features $h_{x-y}$ of edge $e(x,y)$. We believe they will guide GNN model to choose information of neighbor nodes. 

In our experiments, both dual-encoder and cross-encoder use [CLS] representations as embeddings.

\subsection{GNN on Query-passage Graph} \label{3.3}
The most straightforward way to fuse query (passage) information into passage (query) embeddings is directly adding query (passage) embeddings to passage (query) embeddings. However, not all information is effective. Ideally, a model can choose what information to utilize and how much such information should be retained, which is exactly what our proposed model (Figure~\ref{fig:model}) does. Since GAT \cite{velivckovic2018graph} can learn the attention weights to neighbors (i.e., how to choose information of neighbors), it suits well to our work. In our graph, two nodes connected are considered to be relevant, so we can utilize GAT to learn how to exchange information between relevant nodes. 

\paratitle{GAT Layer}
We apply multi-head attention in GAT layer. But for simplicity, we only describe the single-head situation below. Let $\mathcal{N}_i$ denote the neighbors of node $i$ in the graph. GAT layer computes the importance of node $j \in \mathcal{N}_i$ to node $i$ as:
\begin{equation}
    e_{ij} = a^\mathrm{T}[W_t h_i||W_s h_j || W_e h_{i-j}],
\end{equation}
where $h_i \in \mathcal{R}^{d_n}$, $h_j \in \mathcal{R}^{d_n}$, $h_{i-j} \in \mathcal{R}^{d_e}$ are the features of node $i$, node $j$ and edge $e(i,j)$, respectively, and $W_t \in \mathcal{R}^{d_n \times d}$, $W_s \in \mathcal{R}^{d_n \times d}$, $W_e \in \mathcal{R}^{d_e \times d}$, $a \in \mathcal{R}^{3d}$ are learnable model parameters, and $||$ is concatenation operation. In our experiments, we set $d_n = d_e = d$ which equals to the dimension of BERT base (\ie 768). Then the attention weight of node $j \in \mathcal{N}_i$ to node $i$ is calculated by the softmax function and LeakyReLU activation function:
\begin{equation}\label{eq:atention}
    \alpha_{ij} = \frac{\exp(\mbox{LeakyReLU}(e_{ij}))}{\sum_{k \in \mathcal{N}_i}\exp(\mbox{LeakyReLU}(e_{ik}))}.
\end{equation}
The final output features for every node can be computed as weighted sum of linear transformed features of neighbor nodes, and optionally adding an activation function $\sigma$:
\begin{equation}\label{eq:gatOutput}
    \widetilde{h_i} = \sigma(\sum_{j\in \mathcal{N}_i}\alpha_{ij}W_s h_j).
\end{equation}

Considering only node features will change after GAT layer, we define the above formulation as: $\widetilde{h_i} = \mbox{GAT}(\{h_j\}_{j \in \mathcal{N}_i})$ for notation simplicity. We use two GAT layers to implement the interaction between nodes, because two-hop neighbors can exactly establish the relation between the queries and between the passages.

\paratitle{Aggregate}
We first get the aggregated contexts of query neighbors via the first GAT layer:
\begin{equation}\label{eq:gat1}
    \widetilde{h_{q_i}} = \mbox{GAT}(\{h_{p_{ij}}\}_{p_{ij} \in P_i} \cup \{h_{q_i}\}),
\end{equation}
where $P_i$ denotes the set of passages retrieved by $q_i$. Then we concatenate the aggregated contexts and query node features, and apply a single linear layer to get \textbf{passage-interactive query embeddings}:
\begin{equation}\label{eq:iqe}
    h_{q_i}' = W_{pq}[\widetilde{h_{q_i}}||h_{q_i}] + b_{pq},
\end{equation}
where $W_{pq} \in \mathcal{R}^{d\times 2d}$ and $b_{pq} \in \mathcal{R}^d$ are weight matrix and weight vector, respectively. Then we get the aggregated contexts of passage neighbors via the second GAT layer:
\begin{equation}
    \widetilde{h_{p_i}} = \mbox{GAT}(\{h_{q_{ij}}'\}_{{q_{ij}} \in Q_i} \cup \{h_{p_i}\}),
\end{equation}
where $Q_i$ denotes the set of queries retrieving $p_i$. 

\paratitle{Filter Gate}
We can not directly incorporate aggregated contexts of passage neighbors into passage embeddings for the noise in them. We utilize filter gate to "clean"\footnote{Since the passage-interactive query embeddings are not directly involved in the similarity calculation, we should keep as much information as possible for the subsequent calculation. Therefore we do not apply the gate structure to filter noise in the passage-interactive query embeddings, and the final gate will filter all the noise.} the aggregated contexts: 
\begin{equation}\label{eq:gate}
    f_{p_i} = \sigma(W_{qp}[\widetilde{h_{p_i}}||h_{p_i}] + b_{qp}),
\end{equation}
where $W_{qp} \in \mathcal{R}^{d\times 2d}$ and $b_{qp} \in \mathcal{R}^d$ are weight matrix and weight vector, respectively and $\sigma$ represents the sigmoid function. We get the final \textbf{query-interactive passage embeddings} as follows:
\begin{equation}
\label{eq:ipe}
    h_{p_i}' = f_{p_i} \cdot \widetilde{h_{p_i}} + h_{p_i}.
\end{equation}
\subsection{Training Procedure} \label{3.4}
In this section, we present the training procedure of our model. Following \citet{qu2021rocketqa} and \citet{ren2021pair}, we first retrieve the top-k candidates of each query from the corpus by DPR~\cite{karpukhin2020dense} and score them by a well-trained cross-encoder $M_{ce}$ to obtain denoised positives and hard negatives to train our initial dual-encoder $M_{de}$. We utilize $M_{de}$ and $M_{ce}$ to construct our query-passage graph, including adding edges, initializing node features and initializing edge features.

We adopt Eq.(\ref{loss}) as our basic loss function to train the dual-encoder (initialized with $M_{de}$) and GNN jointly. For each training step, we randomly sample a subset of training queries $Q_b = \{q_i\}_{i=1}^b$, getting their denoised positives and hard negatives $P_b = P_b^+ \cup P_b^- = \{p_{q_i}^+\}_{i=1}^b \cup \{p_{q_i}^-\}_{i=1}^b$. We compute query-interactive passage embeddings for each passage in $P_b$, and then utilize them and query embeddings to compute similarity and loss:
\begin{gather}\label{eq:gnnsim}
    s_{\mathcal{G}}(q,p) = E_Q(q)^\mathrm{T} \cdot h_p', \\
    L_{\mathcal{G}} = \sum_{q_i \in Q_b}L(q_i,p^+_{q_i},P_b - \{p^+_{q_i}\},s_{\mathcal{G}}). \label{eq:gnnloss}
\end{gather}
In this way, query encoder can learn how to produce query embeddings with interaction information by being involved in the computation of passage-interactive query embeddings and similarity.

Ideally, we need to recompute the node features by dual-encoder at each training step. However, considering efficiency and hardware resources, we utilize cache passage embeddings of $M_{de}$ as passage node features to compute $\widetilde{h_{q_i}}$ in Eq.(\ref{eq:gat1}), while node features in Eq.(\ref{eq:iqe}$\sim$\ref{eq:ipe}) are recomputed by dual-encoder. For retrieval, we utilize the similarity calculated by Eq.(\ref{eq:gnnsim}) as score to rank all passages. 
%Since query-interactive passage embeddings can be pre-computed offline, our online retrieval efficiency is same as dual-encoder.

\paratitle{Masked Graph Training Algorithm} The method presented above is highly susceptible to information leakage in training. Dropping labeled edges is a common trick to avoid leakage information, but it does not suit our task which will be analysed in later experiments. The training queries are involved in graph construction, while test queries are not, which also leads to the gap between training and inference. When constructing graph, positive passage $p_{q_i}^+$ tends to be retrieved by query $q_i$, which may lead $p_{q_i}^+$ focus too much on $q_i$. Based on these considerations, we propose a Masked Graph Training (MGT) Algorithm which is applicable to other tasks suffering the same dilemma. In every epoch, we split the training queries into two parts $Q_g$ and $Q_t$ which are utilized for constructing the graph and training (i.e., masking some nodes in training), respectively. By this means, we alleviate the gap between training and inference . The proportion of query masked $\beta$ in the graph can not be too high, otherwise it will cause the gap between training graph and inference graph. For more details, you can refer to appendix \ref{appendix:algorithm}.

==> EMNLP 2022/section/old_method.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=1.8\columnwidth]{EMNLP 2022/figs/gnn-encoder-v2.pdf}
    \caption{
        Overview of \gmodel.
    }
    \label{fig:model}
\end{figure*}
\section{Methodology}
\subsection{Preliminary}
Given a query $q$, dense retriever is required to retrieve k most relevant passages $\{p_i\}_{i=1}^k$ from a large corpus consisting of hundreds of thousands of passages. For the sake of retrieval efficiency, the dual-encoder architecture is widely adopted, where query encoder $E_Q(\cdot)$ and passage encoder $E_P(\cdot)$ are used to embed query $q$ and passage $p$ into $d$-dimensional vectors respectively. The similarity between query $q$ and passage $p$ can be computed as the dot product of their vectors:
\begin{equation}
    s(q,p) = E_Q(q)^\mathrm{T}\cdot E_P(p).
\end{equation}

The training objective of the dual-encoder is to learn embeddings of queries and passages to make positive query-passage pairs have higher similarity than the negative query-passage pairs in training data. Hence, the contrastive-learning loss function is adopted for the dual-encoder:
\begin{equation}\label{loss}
     \begin{aligned}
    &L(q,p^+,\{p^-\},s) = \\
    &- \log \frac{e^{s(q,p^+)}}{e^{s(q,p^+)}+\sum_{\{p^-\}}e^{s(q,p^-)}},
    \end{aligned}
\end{equation}
where $q$ and $p^+$ represent query and positive passage respectively, and $\{p^-\}$ represents the set of negative passages.

In practical retrieval systems, passage embeddings are usually pre-computed offline, while query embeddings are computed by the query encoder in an ad hoc manner. Therefore we can obtain better passage embeddings through a complicated encoder as long as it does not increase the online inference latency.
\subsection{Query-passage Graph}
In \gmodel, we incorporate query information into passage embeddings based on Graph Attention Network (GAT) \cite{velivckovic2018graph}. GAT learns how to interact with neighbor nodes which can be utilized to exchange information between queries and passages.

\paratitle{Graph Construction} \label{3.2} We use all the passages $P = \{p_i\}_{i=1}^m$ and training queries 
$Q = \{q_i\}_{i=1}^n$ as nodes to construct our query-passage graph, where $n$ and $m$ denote the number of training queries and passages, respectively. Let $\mathcal{G} = (\mathcal{V},\mathcal{E})$ denote our graph, which consists of a node set $\mathcal{V} = \mathcal{V}_q \cup \mathcal{V}_p$ and an edge set $\mathcal{E} = \mathcal{E}_{pp} \cup \mathcal{E}_{pq} \cup \mathcal{E}_{qq}$. 
$\mathcal{V}_p$ and $\mathcal{V}_q$ denote the passage node set and the query node set, respectively. $\mathcal{E}_{pp}$, $\mathcal{E}_{pq}$, and $\mathcal{E}_{qq}$ denote the edges between passage nodes, between passage nodes and query nodes, and between query nodes, respectively. 
The edge between node $x$ and node $y$ is denoted as $e(x,y)$.

We retrieve the top-k candidate passages $P_i = \{p_{ij}\}_{j=1}^k$ for each query $q_i$ from the corpus by the dual-encoder. We add edges between $q_i$ and each passage $p_{ij}$ in the top-k retrieved passages $P_i$ which may be relevant to $q_i$. These edges compose $\mathcal{E}_{pq}$ (i.e., $\mathcal{E}_{pq} = \{e(q_i,p_{i_j})\}_{i=1,j=1}^{n,k}$). Since we can not directly distinguish whether there is relation between the queries and between the passages, we only add self-loops to each passage and query (i.e., $\mathcal{E}_{pp}=\{e(p_i,p_i)\}_{i=1}^m$ and $\mathcal{E}_{qq}=\{e(q_i,q_i)\}_{i=1}^n$). To summarize, our graph $\mathcal{G}$ has a total of $(n+m)$ nodes and $(n\times k + m +n)$ edges.

\paratitle{GAT Layer}
Similar to Transformer \cite{vaswani2017attention}, we apply multi-head attention mechanism in GAT layer. But for simplicity, we only describe the single-head situation below. Let $\mathcal{N}_i$ denote the neighbors of node $i$ in the graph. GAT layer computes the importance of node $j \in \mathcal{N}_i$ to node $i$ as:
\begin{equation}
    e_{ij} = a^\mathrm{T}[W_t h_i||W_s h_j || W_e h_{i-j}],
\end{equation}
where $h_i \in \mathcal{R}^{d_n}$, $h_j \in \mathcal{R}^{d_n}$, $h_{i-j} \in \mathcal{R}^{d_e}$ are the features of node $i$, node $j$ and edge $e(i,j)$, respectively, and $W_t \in \mathcal{R}^{d_n \times d}$, $W_s \in \mathcal{R}^{d_n \times d}$, $W_e \in \mathcal{R}^{d_e \times d}$, $a \in \mathcal{R}^{3d}$ are learnable model parameters, and $||$ is concatenation operation. In our experiments, we set $d_n = d_e = d$ which equals to the dimension of BERT base (\ie 768). Then the attention weight of node $j \in \mathcal{N}_i$ to node $i$ is calculated by the softmax function and LeakyReLU activation function:
\begin{equation}\label{eq:atention}
    \alpha_{ij} = \frac{\exp(\mbox{LeakyReLU}(e_{ij}))}{\sum_{k \in \mathcal{N}_i}\exp(\mbox{LeakyReLU}(e_{ik}))}.
\end{equation}
The final output features for every node can be computed as weighted sum of linear transformed features of neighbor nodes, and optionally adding an activation function $\sigma$:
\begin{equation}\label{eq:gatOutput}
    \widetilde{h_i} = \sigma(\sum_{j\in \mathcal{N}_i}\alpha_{ij}W_s h_j).
\end{equation}

Considering only node features will change after GAT layer, we define the above formulation as: $\widetilde{h_i} = \mbox{GAT}(\{h_j\}_{j \in \mathcal{N}_i})$ for notation simplicity. 
\subsection{Query-interactive Passage embeddings} \label{3.3}
The most straightforward way to incorporate query information into passage embeddings is directly adding query embeddings to passage embeddings. However, not all query information is effective. Ideally, a model can choose what query information to utilize and how much such information should be retained, which is exactly what our proposed model does.

Since GAT can learn the attention weights to neighbor nodes (i.e., how to choose information of neighbor nodes), it suits well to our work. In our graph, two nodes connected are considered to be relevant, so we can utilize GAT to learn how to exchange information between relevant nodes. We use two GAT layers to implement the interactions between nodes, because two-hop neighbors can exactly establish the relation between the queries and between the passages. We use the dual-encoder to get query embeddings $h_{q_i} = E_Q(q_i) \in \mathcal{R}^d$and passage embeddings $h_{p_i} = E_P(p_i) \in \mathcal{R}^d$ as our graph node features. Since the cross-encoder can better capture the interactive information between text pairs, we utilize the embeddings of text pairs $(x,y)$ by the cross-encoder as the edge features $h_{x-y}\in \mathcal{R}^d$. We believe it will guide model to choose information of neighbor nodes. In our experiments, both dual-encoder and cross-encoder use [CLS] representations as text embeddings.

We first get the aggregated contexts of query neighbors via the first GAT layer:
\begin{equation}\label{eq:gat1}
    \widetilde{h_{q_i}} = \mbox{GAT}(\{h_{p_{ij}}\}_{p_{ij} \in P_i} \cup \{h_{q_i}\}),
\end{equation}
where $P_i$ denotes the set of passages retrieved by $q_i$. Then we concatenate the aggregated contexts and query node features, and apply a single linear layer to get passage-interactive query embeddings:
\begin{equation}
    h_{q_i}' = W_{pq}[\widetilde{h_{q_i}}||h_{q_i}] + b_{pq},
\end{equation}
where $W_{pq} \in \mathcal{R}^{d\times 2d}$ and $b_{pq} \in \mathcal{R}^d$ are weight matrix and weight vector, respectively. Then we get the aggregated contexts of passage neighbors via the second GAT layer:
\begin{equation}
    \widetilde{h_{p_i}} = \mbox{GAT}(\{h_{q_{ij}}'\}_{{q_{ij}} \in Q_i} \cup \{h_{p_i}\}),
\end{equation}
where $Q_i$ denotes the set of queries which retrieve $p_i$. We can not directly incorporate aggregated contexts of passage neighbors into passage embeddings for the noise in it. We utilize the gate structure in Long Short-Term Memory \cite{hochreiter1997long}:
\begin{equation}\label{eq:gate}
    f_{p_i} = \sigma(W_{qp}[\widetilde{h_{p_i}}||h_{p_i}] + b_{qp}),
\end{equation}
where $W_{qp} \in \mathcal{R}^{d\times 2d}$ and $b_{qp} \in \mathcal{R}^d$ are weight matrix and weight vector, respectively and $\sigma$ represents the sigmoid function, to "clean"\footnote{Since the passage-interactive query embeddings are not directly involved in the similarity calculation, we should keep as much information as possible for the subsequent calculation. Therefore we do not apply the gate structure to filter noise in the interactive query embeddings, and the final gate will filter all the noise} the aggregated contexts. We get the final query-interactive passage embeddings as follows:
\begin{equation}
\label{eq:ipe}
    h_{p_i}' = f_{p_i} \cdot \widetilde{h_{p_i}} + h_{p_i}.
\end{equation}
\subsection{Training Procedure} \label{3.4}
In this section, we present the training procedure of our model. Following \citet{qu2021rocketqa} and \citet{ren2021pair}, we first retrieve the top-k candidates of each query from the corpus by DPR~\cite{karpukhin2020dense} and score them by a well-trained cross-encoder $M_{ce}$ to obtain denoised positives and hard negatives to train our initial dual-encoder $M_{de}$. We utilize $M_{de}$ and $M_{ce}$ to construct our query-passage graph, including adding edges, initializing node features and initializing edge features.

We adopt Eq.(\ref{loss}) as our basic loss function to train the dual-encoder (initialized with $M_{de}$) and GNN jointly. For each training step, we randomly sample a subset of training queries $Q_b = \{q_i\}_{i=1}^b$, getting their denoised positives and hard negatives $P_b = P_b^+ \cup P_b^- = \{p_{q_i}^+\}_{i=1}^b \cup \{p_{q_i}^-\}_{i=1}^b$. We compute query-interactive passage embeddings for each passage in $P_b$, and then utilize them and query embeddings to compute similarity and loss:
\begin{gather}\label{eq:gnnsim}
    s_{\mathcal{G}}(q,p) = E_Q(q)^\mathrm{T} \cdot h_p', \\
    L_{\mathcal{G}} = \sum_{q_i \in Q_b}L(q_i,p^+_{q_i},P_b - \{p^+_{q_i}\},s_{\mathcal{G}}). \label{eq:gnnloss}
\end{gather}

Ideally, we need to recompute the node features by dual-encoder at each training step. However, considering efficiency and hardware resources, we utilize cache passage embeddings of $M_{de}$ as passage node features to compute the aggregated contexts of passage neighbors $\widetilde{h_{p_i}}$. Passage embeddings $h_{p_i}$ in Eq.(\ref{eq:gate}) and Eq.(\ref{eq:ipe}) will be recomputed by passage encoder. For retrieval, we utilize the similarity calculated by Eq.(\ref{eq:gnnsim}) as score to rank all passages. Since query-interactive passage embeddings can be pre-computed offline, our online retrieval efficiency is same as dual-encoder.

\paratitle{Masked Graph Training Algorithm} The method presented above is highly susceptible to information leakage in training. Dropping labeled edges is a common trick to avoid leakage information, but it does not suit our task which will be analysed in later experiments. The training queries are involved in graph construction, while test queries are not, which also leads to the gap between training and inference. When constructing graph, positive passage $p_{q_i}^+$ tends to be retrieved by query $q_i$, which may lead $p_{q_i}^+$ focus too much on $q_i$. Based on these considerations, we propose a Masked Graph Training Algorithm which is applicable to other tasks suffering the same dilemma. In every epoch, we split the training queries into two parts $Q_g$ and $Q_t$ which are utilized for constructing the graph and training GAT layers (i.e., masking some nodes in training), respectively. By this means, we alleviate the gap between training and inference . The proportion of query masked $\beta$ in the graph can not be too high, otherwise it will cause the gap between training graph and inference graph. For more details, you can refer to appendix \ref{appendix:algorithm}.

==> EMNLP 2022/section/related_work.tex <==
\pdfoutput=1
\section{Related Work}
Our work touches on two strands of research within dense passage retrieval and graph neural network. 
%In this section, we will review the existing work related with the passage retrieval and graph neural network. 
% It's noteworthy that GNN is 

\subsection{Dense Passage Retrieval}
%Without loss of generality, the passage retrieval approaches can be classified into two categories including sparse retrieval and dense retrieval. Traditional sparse approaches~\cite{traditionalqa} implement term-based retriever by weighting the terms based on their frequency information(e.g. TF-IDF and BM25) or semantic information~\citet{dai2019deepct, nogueira2019doc2query, Nogueira2019docTTTTTquery}.
%, which have limited representation capabilities. 
%Recently, pre-trained language models are utilized to weight or augment the document/query terms to incorporate semantic information~\citet{dai2019deepct, nogueira2019doc2query, Nogueira2019docTTTTTquery}.
%\citet{dai2019deepct} uses BERT to learn the term weight. Both doc2query~\cite{nogueira2019doc2query} and docTTTTTquery~\cite{Nogueira2019docTTTTTquery} employ query generation to expand documents. 

%Different from the above term-based sparse retrieval approaches, the dense retrieval approaches have been proposed to map both questions and documents to continuous vectors (i.e., embeddings).
The dense passage retrieval approaches have been proposed to map both questions and documents to continuous vectors (i.e., embeddings), which has achieved better performance than sparse retrieval approaches~\cite{traditionalqa, dai2019deepct}.
%Models like DSSM~\cite{huang2013dssm}, CLSM~\cite{shen2014clsm}, ARC-I~\cite{hu2014convolutionalARCI} and QALSTM~\cite{tan2015QALSTM} learn continuous document representations based on different network architectures, such as fully connection, CNN and RNN. 
%After the network, a simple matching function such as cosine similarity are used to calculate similarity scores. 
%These models encode the query and document independently thus are applicable for the first-stage.
%Recently, pre-trained language models such as BERT~\cite{BERT} have shown great success when fine-tuned on downstream tasks. Dense retrieval approaches also tend to make use of the PLMs.
Existing approaches can be roughly divided into two categories: pre-training and fine-tuning. The first type of methods often explores pre-training objectives/architectures designed for retrieval.
~\citet{lee2019ICT} pre-trains the retriever with an unsupervised Inverse Cloze Task (ICT). Condenser~\cite{gao2021condenser} proposes a dense retrieval pre-training architecture which learns to condense information into the dense vector through LM pre-training. coCondenser~\cite{gao2021unsupervised} adds an unsupervised corpus-level contrastive
loss on top of the Condenser~\cite{gao2021condenser} to warm up passage embeddings.
%A sentence is treated as a pseudo question and its context is treated as pseudo evidence. Given a pseudo-question, ICT requires selecting the corresponding pseudo-evidence out of the candidates in a batch. The retriever and the reader are trained jointly. 
%~\citet{guu2020realm} augments language model pre-training process with a latent knowledge retriever, which allows the model to retrieve and attend over documents from a large corpus such as Wikipedia. 
%\citet{MaWSDM21PROP}  proposes Pre-training with Representative wOrds Prediction (PROP) for ad-hoc retrieval.
%which assumes that the query is generated as the piece of text representative of the "ideal" document. 

The second type of methods often fine-tunes pre-trained language models on labeled data. ~\citet{karpukhin2020dense} proposes a dense embedding model using only pairs of questions and passages, without additional pre-training. \citet{xiong2020approximate, qu2021rocketqa} identify that the negative samples during training may not be representative, thus mechanism of selecting hard training negatives is designed. ~\citet{khattab2020colbert, Humeau2019polyencoder} incorporate late interaction architectures into the learning process that independently encode the query and the document firstly. 
%They employ a cheap yet powerful interaction step such as MaxSim and attention network, that models fine-grained similarity of the query and the passage to improve the performance. 
\citet{tang2021Pseudo} 
%address the problem of serious information loss during the encoding of documents since the queries are agnostic in dual-encoder. They 
designs a method to mimic the queries on each of the documents by clustering to enhance the document representation.
PAIR \cite{ren2021pair} leverages passage-centric similarity relation into training object to discriminate between positive and negative passages.
RocketQAv2 \cite{renrocketqav2} introduces dynamic listwise distillation to jointly train retriever and re-ranker.
%and represent the documents by multiple pseudo queries. 
%rocketqav2 PAIR
%Our work follows the second class of fine-tuning methods, which show better performance with less cost.

\begin{figure*}
    \centering
    \includegraphics[width=2.0\columnwidth]{EMNLP 2022/figs/gnn-encoder-v2.pdf}
    \caption{
        Overview of \gmodel which can be divided into three parts: (1) Dual-encoder; (2) Cross-encoder; (3) GNN on query-passage graph. Node and edge features of query-passage graph are initialized by dual-encoder and cross-encoder, respectively. Only the parameters of dual-encoder and GNN will be updated during training.
    }
    \label{fig:model}
\end{figure*}

\subsection{Graph Neural Network}
Graph neural network (GNN) captures the relationships between nodes connected with edges, which propagates features across nodes layer by layer~\cite{scarselli2008gnn}. Graph attention network (GAT)~\cite{velivckovic2018graph} leverages masked self-attentional layers to address the shortcomings of prior work based on graph convolutions or their approximations. GNN has demonstrated effectiveness in a wide variety of tasks such as text classification \cite{lin2021bertgcn}, question answering ~\cite{de2018qagcn},  recommendation~\cite{wu2019recommendationgcn} and relation extraction~\cite{li2020REgraph}. For example, %Star-Transformer~\cite{star-transformer} reduces the computation complexity of the standard Transformer by replacing the fully-connected structure in self-attention with a star-like topology. 
~\citet{QAGNN} connects the question-answering context and knowledge graph to form a joint graph, and mutually updates their representations to perform joint reasoning over the language and the knowledge graph. 
%We also list some researches that combine graphs and pre-trained models, although little research has been done on this.

Compared to existing work, our work serves the dense passage retrieval and presents a novel fine-tuning method to fuse query (passage) information into passage (query) embeddings via GNN. 
%The interaction information between the query and the passage is captured during the passage (query) encoding process.


==> EMNLP 2022/table/ablation.tex <==
\begin{table}[!t]
\centering
\begin{adjustbox}{max width=\linewidth}
%  \begin{tabular}{p{3.3cm}cccccccccc}
    \begin{tabular}{lcccccccccc}
    \toprule
    Methods & R@5 & R@20 & R@100 \\
    \midrule
    \gmodel & \textbf{76.8} & \textbf{84.9} & \textbf{89.3} \\
    \midrule
    w/o GNN & 75.1 & 83.6 & 89.1 \\
    w/o MGT & 76.0 & 84.4 & 89.1 \\
    w/o filter gate &  76.3 & 84.6 & 89.2  \\
    w/o edge features & 76.5 & 84.7 & 89.2 \\
    w/ one layer & 76.3 & 84.5 & 89.2 \\
  \bottomrule
\end{tabular}
\end{adjustbox}
  \caption{Ablation study of different components of \gmodel on Natural Questions. 
  }
  \label{tab:ablation}
\end{table}

==> EMNLP 2022/table/efficiency.tex <==
\begin{table}[t]
\centering
  \begin{tabular}{p{2.5cm}cccccccccc}
    \toprule
    Methods & Doc Encoding & Retrieval \\
    \midrule
    DPR & 0.41ms & 1.9ms \\
    ColBERT & 0.41ms & 90ms \\
    RocketQAv2 & 0.41ms & 1.9ms \\
    \gmodel & 0.46ms & 1.9ms \\
  \bottomrule
\end{tabular}
  \caption{Time cost of online retrieval and offline document encoding for Natural Questions test set.}
  \label{tab:effic}
\end{table}

==> EMNLP 2022/table/main_result.tex <==
\begin{table*}[htp]
\centering
  \begin{tabular}{p{3cm}lccccccc}
    \toprule
    \multirow{2}{*}{\textbf{Methods}} & \multirow{2}{*}{\textbf{PLM}} & \multicolumn{3}{c}{\textbf{MSMARCO Dev}} &
    \multicolumn{3}{c}{\textbf{Natural Questions Test}} &\\
    & & MRR@10 & R@50 & R@1000 & R@5 & R@20 & R@100 \\
    \midrule
    BM25~(anserini) & - & 18.7 & 59.2 & 85.7 & - & 59.1 & 73.7\\
    \midrule
    % doc2query & - & 21.5 & 64.4 & 89.1 & - & - & - \\
    DeepCT & - & 24.3 & 69.0 & 91.0 & - & - & - \\
    % docTTTTTquery & - & 27.7 & 75.6 & 94.7 & - & - & - \\
    GAR & - & - & - & - & - & 74.4 & 85.3 \\
    COIL & - & 35.5 & - & 96.3 & - & - & - \\
    \midrule
    DPR (single) & BERT$_{\rm base}$ & - & - & - & - & 78.4 & 85.4 \\
    ANCE (single) & RoBERTa$_{\rm base}$ & 33.0 & - & 95.9 & - & 81.9 & 87.5 \\
    ColBERT  & BERT$_{\rm base}$ & 36.0 & 82.9 & 96.8 & - & - & - \\
    NPRINC & BERT$_{\rm base}$ & 31.1 & - & 97.7 & 73.3 & 82.8 & 88.4 \\
    RocketQA  & ERNIE$_{\rm base}$ & 37.0 & 85.5 & 97.9 & 74.0 & 82.7 & 88.5  \\
    PAIR  & ERNIE$_{\rm base}$ & 37.9 & 86.4 & 98.2 & 74.9 & 83.5 & 89.1 \\
    Condenser$^\dagger$ & - & 36.6 & - & 97.4 & - & 83.2 & 88.4 \\
    RocketQAv2  & ERNIE$_{\rm base}$ & 38.8 & 86.2 & 98.1 & 75.1 & 83.7 & 89.0\\
    coCondenser$^\dagger$ & - & 38.2 & - & \textbf{98.4} & 75.8 & 84.3 & 89.0 \\
    \midrule
   \gmodel & ERNIE$_{\rm base}$ & \textbf{39.3} & \textbf{86.9} & 98.3 & \textbf{76.8} & \textbf{84.9} & \textbf{89.3} \\
  \bottomrule
\end{tabular}
 \caption{Experimental results on MSMARCO dev set and Natural Questions test set. We copy the results from original papers, while leaving it blank if unavailable. The best results are marked bold. $^\dagger$Note that Condenser and coCondenser are pre-training methods.}
\label{tab:mainR}
\end{table*}

==> EMNLP 2022/table/trivia_result.tex <==
\begin{table}[t]
\centering
  \begin{tabular}{p{2.8cm}cccccccccc}
    \toprule
    Methods & R@5 & R@20 & R@100 \\
    \midrule
    BM25~(anserini) & - & 66.9 & 76.7 \\
    DPR (single) & - & 79.4 & 85.0  \\
    ANCE (single) & - &80.3 & 85.3 \\
    GAR & 73.1 & 80.4 & 85.7 \\
    PAIR & 76.3$^*$ & 82.4$^*$ & 86.9$^*$ \\
    Condenser &  - & 81.9 & 86.2 \\
    RocketQAv2 & 76.4$^*$ & 82.6$^*$ & 86.7$^*$ \\
    coCondenser & 76.8 & 83.2 & \textbf{87.3} \\
    \midrule
    \gmodel & \textbf{77.7} & \textbf{83.3} & 87.2 \\
  \bottomrule
\end{tabular}
  \caption{Experimental results on TriviaQA test set. The results of PAIR and RocketQAv2 are reproduced (marked with $^*$), while others are copied from the original paper. All dense retrieval models are initialized with BERT$_{\rm base}$. 
  % The best results are marked bold and unavailable results are left blank.
  }
  \label{tab:triviaR}
\end{table}

==> section/old_method.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=1.8\columnwidth]{EMNLP 2022/figs/gnn-encoder-v2.pdf}
    \caption{
        Overview of \gmodel.
    }
    \label{fig:model}
\end{figure*}
\section{Methodology}
\subsection{Preliminary}
Given a query $q$, dense retriever is required to retrieve k most relevant passages $\{p_i\}_{i=1}^k$ from a large corpus consisting of hundreds of thousands of passages. For the sake of retrieval efficiency, the dual-encoder architecture is widely adopted, where query encoder $E_Q(\cdot)$ and passage encoder $E_P(\cdot)$ are used to embed query $q$ and passage $p$ into $d$-dimensional vectors respectively. The similarity between query $q$ and passage $p$ can be computed as the dot product of their vectors:
\begin{equation}
    s(q,p) = E_Q(q)^\mathrm{T}\cdot E_P(p).
\end{equation}

The training objective of the dual-encoder is to learn embeddings of queries and passages to make positive query-passage pairs have higher similarity than the negative query-passage pairs in training data. Hence, the contrastive-learning loss function is adopted for the dual-encoder:
\begin{equation}\label{loss}
     \begin{aligned}
    &L(q,p^+,\{p^-\},s) = \\
    &- \log \frac{e^{s(q,p^+)}}{e^{s(q,p^+)}+\sum_{\{p^-\}}e^{s(q,p^-)}},
    \end{aligned}
\end{equation}
where $q$ and $p^+$ represent query and positive passage respectively, and $\{p^-\}$ represents the set of negative passages.

In practical retrieval systems, passage embeddings are usually pre-computed offline, while query embeddings are computed by the query encoder in an ad hoc manner. Therefore we can obtain better passage embeddings through a complicated encoder as long as it does not increase the online inference latency.
\subsection{Query-passage Graph}
In \gmodel, we incorporate query information into passage embeddings based on Graph Attention Network (GAT) \cite{velivckovic2018graph}. GAT learns how to interact with neighbor nodes which can be utilized to exchange information between queries and passages.

\paratitle{Graph Construction} \label{3.2} We use all the passages $P = \{p_i\}_{i=1}^m$ and training queries 
$Q = \{q_i\}_{i=1}^n$ as nodes to construct our query-passage graph, where $n$ and $m$ denote the number of training queries and passages, respectively. Let $\mathcal{G} = (\mathcal{V},\mathcal{E})$ denote our graph, which consists of a node set $\mathcal{V} = \mathcal{V}_q \cup \mathcal{V}_p$ and an edge set $\mathcal{E} = \mathcal{E}_{pp} \cup \mathcal{E}_{pq} \cup \mathcal{E}_{qq}$. 
$\mathcal{V}_p$ and $\mathcal{V}_q$ denote the passage node set and the query node set, respectively. $\mathcal{E}_{pp}$, $\mathcal{E}_{pq}$, and $\mathcal{E}_{qq}$ denote the edges between passage nodes, between passage nodes and query nodes, and between query nodes, respectively. 
The edge between node $x$ and node $y$ is denoted as $e(x,y)$.

We retrieve the top-k candidate passages $P_i = \{p_{ij}\}_{j=1}^k$ for each query $q_i$ from the corpus by the dual-encoder. We add edges between $q_i$ and each passage $p_{ij}$ in the top-k retrieved passages $P_i$ which may be relevant to $q_i$. These edges compose $\mathcal{E}_{pq}$ (i.e., $\mathcal{E}_{pq} = \{e(q_i,p_{i_j})\}_{i=1,j=1}^{n,k}$). Since we can not directly distinguish whether there is relation between the queries and between the passages, we only add self-loops to each passage and query (i.e., $\mathcal{E}_{pp}=\{e(p_i,p_i)\}_{i=1}^m$ and $\mathcal{E}_{qq}=\{e(q_i,q_i)\}_{i=1}^n$). To summarize, our graph $\mathcal{G}$ has a total of $(n+m)$ nodes and $(n\times k + m +n)$ edges.

\paratitle{GAT Layer}
Similar to Transformer \cite{vaswani2017attention}, we apply multi-head attention mechanism in GAT layer. But for simplicity, we only describe the single-head situation below. Let $\mathcal{N}_i$ denote the neighbors of node $i$ in the graph. GAT layer computes the importance of node $j \in \mathcal{N}_i$ to node $i$ as:
\begin{equation}
    e_{ij} = a^\mathrm{T}[W_t h_i||W_s h_j || W_e h_{i-j}],
\end{equation}
where $h_i \in \mathcal{R}^{d_n}$, $h_j \in \mathcal{R}^{d_n}$, $h_{i-j} \in \mathcal{R}^{d_e}$ are the features of node $i$, node $j$ and edge $e(i,j)$, respectively, and $W_t \in \mathcal{R}^{d_n \times d}$, $W_s \in \mathcal{R}^{d_n \times d}$, $W_e \in \mathcal{R}^{d_e \times d}$, $a \in \mathcal{R}^{3d}$ are learnable model parameters, and $||$ is concatenation operation. In our experiments, we set $d_n = d_e = d$ which equals to the dimension of BERT base (\ie 768). Then the attention weight of node $j \in \mathcal{N}_i$ to node $i$ is calculated by the softmax function and LeakyReLU activation function:
\begin{equation}\label{eq:atention}
    \alpha_{ij} = \frac{\exp(\mbox{LeakyReLU}(e_{ij}))}{\sum_{k \in \mathcal{N}_i}\exp(\mbox{LeakyReLU}(e_{ik}))}.
\end{equation}
The final output features for every node can be computed as weighted sum of linear transformed features of neighbor nodes, and optionally adding an activation function $\sigma$:
\begin{equation}\label{eq:gatOutput}
    \widetilde{h_i} = \sigma(\sum_{j\in \mathcal{N}_i}\alpha_{ij}W_s h_j).
\end{equation}

Considering only node features will change after GAT layer, we define the above formulation as: $\widetilde{h_i} = \mbox{GAT}(\{h_j\}_{j \in \mathcal{N}_i})$ for notation simplicity. 
\subsection{Query-interactive Passage embeddings} \label{3.3}
The most straightforward way to incorporate query information into passage embeddings is directly adding query embeddings to passage embeddings. However, not all query information is effective. Ideally, a model can choose what query information to utilize and how much such information should be retained, which is exactly what our proposed model does.

Since GAT can learn the attention weights to neighbor nodes (i.e., how to choose information of neighbor nodes), it suits well to our work. In our graph, two nodes connected are considered to be relevant, so we can utilize GAT to learn how to exchange information between relevant nodes. We use two GAT layers to implement the interactions between nodes, because two-hop neighbors can exactly establish the relation between the queries and between the passages. We use the dual-encoder to get query embeddings $h_{q_i} = E_Q(q_i) \in \mathcal{R}^d$and passage embeddings $h_{p_i} = E_P(p_i) \in \mathcal{R}^d$ as our graph node features. Since the cross-encoder can better capture the interactive information between text pairs, we utilize the embeddings of text pairs $(x,y)$ by the cross-encoder as the edge features $h_{x-y}\in \mathcal{R}^d$. We believe it will guide model to choose information of neighbor nodes. In our experiments, both dual-encoder and cross-encoder use [CLS] representations as text embeddings.

We first get the aggregated contexts of query neighbors via the first GAT layer:
\begin{equation}\label{eq:gat1}
    \widetilde{h_{q_i}} = \mbox{GAT}(\{h_{p_{ij}}\}_{p_{ij} \in P_i} \cup \{h_{q_i}\}),
\end{equation}
where $P_i$ denotes the set of passages retrieved by $q_i$. Then we concatenate the aggregated contexts and query node features, and apply a single linear layer to get passage-interactive query embeddings:
\begin{equation}
    h_{q_i}' = W_{pq}[\widetilde{h_{q_i}}||h_{q_i}] + b_{pq},
\end{equation}
where $W_{pq} \in \mathcal{R}^{d\times 2d}$ and $b_{pq} \in \mathcal{R}^d$ are weight matrix and weight vector, respectively. Then we get the aggregated contexts of passage neighbors via the second GAT layer:
\begin{equation}
    \widetilde{h_{p_i}} = \mbox{GAT}(\{h_{q_{ij}}'\}_{{q_{ij}} \in Q_i} \cup \{h_{p_i}\}),
\end{equation}
where $Q_i$ denotes the set of queries which retrieve $p_i$. We can not directly incorporate aggregated contexts of passage neighbors into passage embeddings for the noise in it. We utilize the gate structure in Long Short-Term Memory \cite{hochreiter1997long}:
\begin{equation}\label{eq:gate}
    f_{p_i} = \sigma(W_{qp}[\widetilde{h_{p_i}}||h_{p_i}] + b_{qp}),
\end{equation}
where $W_{qp} \in \mathcal{R}^{d\times 2d}$ and $b_{qp} \in \mathcal{R}^d$ are weight matrix and weight vector, respectively and $\sigma$ represents the sigmoid function, to "clean"\footnote{Since the passage-interactive query embeddings are not directly involved in the similarity calculation, we should keep as much information as possible for the subsequent calculation. Therefore we do not apply the gate structure to filter noise in the interactive query embeddings, and the final gate will filter all the noise} the aggregated contexts. We get the final query-interactive passage embeddings as follows:
\begin{equation}
\label{eq:ipe}
    h_{p_i}' = f_{p_i} \cdot \widetilde{h_{p_i}} + h_{p_i}.
\end{equation}
\subsection{Training Procedure} \label{3.4}
In this section, we present the training procedure of our model. Following \citet{qu2021rocketqa} and \citet{ren2021pair}, we first retrieve the top-k candidates of each query from the corpus by DPR~\cite{karpukhin2020dense} and score them by a well-trained cross-encoder $M_{ce}$ to obtain denoised positives and hard negatives to train our initial dual-encoder $M_{de}$. We utilize $M_{de}$ and $M_{ce}$ to construct our query-passage graph, including adding edges, initializing node features and initializing edge features.

We adopt Eq.(\ref{loss}) as our basic loss function to train the dual-encoder (initialized with $M_{de}$) and GNN jointly. For each training step, we randomly sample a subset of training queries $Q_b = \{q_i\}_{i=1}^b$, getting their denoised positives and hard negatives $P_b = P_b^+ \cup P_b^- = \{p_{q_i}^+\}_{i=1}^b \cup \{p_{q_i}^-\}_{i=1}^b$. We compute query-interactive passage embeddings for each passage in $P_b$, and then utilize them and query embeddings to compute similarity and loss:
\begin{gather}\label{eq:gnnsim}
    s_{\mathcal{G}}(q,p) = E_Q(q)^\mathrm{T} \cdot h_p', \\
    L_{\mathcal{G}} = \sum_{q_i \in Q_b}L(q_i,p^+_{q_i},P_b - \{p^+_{q_i}\},s_{\mathcal{G}}). \label{eq:gnnloss}
\end{gather}

Ideally, we need to recompute the node features by dual-encoder at each training step. However, considering efficiency and hardware resources, we utilize cache passage embeddings of $M_{de}$ as passage node features to compute the aggregated contexts of passage neighbors $\widetilde{h_{p_i}}$. Passage embeddings $h_{p_i}$ in Eq.(\ref{eq:gate}) and Eq.(\ref{eq:ipe}) will be recomputed by passage encoder. For retrieval, we utilize the similarity calculated by Eq.(\ref{eq:gnnsim}) as score to rank all passages. Since query-interactive passage embeddings can be pre-computed offline, our online retrieval efficiency is same as dual-encoder.

\paratitle{Masked Graph Training Algorithm} The method presented above is highly susceptible to information leakage in training. Dropping labeled edges is a common trick to avoid leakage information, but it does not suit our task which will be analysed in later experiments. The training queries are involved in graph construction, while test queries are not, which also leads to the gap between training and inference. When constructing graph, positive passage $p_{q_i}^+$ tends to be retrieved by query $q_i$, which may lead $p_{q_i}^+$ focus too much on $q_i$. Based on these considerations, we propose a Masked Graph Training Algorithm which is applicable to other tasks suffering the same dilemma. In every epoch, we split the training queries into two parts $Q_g$ and $Q_t$ which are utilized for constructing the graph and training GAT layers (i.e., masking some nodes in training), respectively. By this means, we alleviate the gap between training and inference . The proportion of query masked $\beta$ in the graph can not be too high, otherwise it will cause the gap between training graph and inference graph. For more details, you can refer to appendix \ref{appendix:algorithm}.

==> table/data_statistics.tex <==
\begin{table}[!t]
\centering
\tabcolsep=0.12cm
\begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{lcccc}
    \toprule
    \bf Datasest & \bf \#q in train & \bf \#q in dev & \bf \#q in test & \bf \#p \\
    \midrule
    MSMARCO & 502,939 & 6,980 & 6,837 & 8,841,823\\
    NQ & 79,168 & 8,757 & 3,610 & 21,015,324\\
    TQA &  78,785 & 8,837 & 11,313 & 21,015,324\\
  \bottomrule
\end{tabular}
\end{adjustbox}
  \caption{The statistics of datasets MSMARCO, NQ and TQA. Here, \#q and \#p denote the number of query in set and all passage.
  }
  \label{tab:data_statistics}
\end{table}
